Exactly Hittable Interval Graphs

Given a set system $\mathcal{X} = \{\mathcal{U},\mathcal{S}\}$, where $\mathcal{U}$ is a set of elements and $\mathcal{S}$ is a set of subsets of $\mathcal{U}$, an exact hitting set $\mathcal{U}'$ is a subset of $\mathcal{U}$ such that each subset in $\mathcal{S}$ contains exactly one element in $\mathcal{U}'$. We refer to a set system as exactly hittable if it has an exact hitting set. In this paper, we study interval graphs which have intersection models that are exactly hittable. We refer to these interval graphs as exactly hittable interval graphs (EHIG). We present a forbidden structure characterization for EHIG. We also show that the class of proper interval graphs is a strict subclass of EHIG. Finally, we give an algorithm that runs in polynomial time to recognize graphs belonging to the class of EHIG.

==> input/gadgetAndMinCliqueCover.tex <==
%The big figure begins
\begin{figure}[ht]
\centering
% \begin{tikzpicture}[scale=0.8, every node/.style={scale=0.8}]
% \node (D1) at (7.5,-3.3){};
% \node (D2) at (9.7,-3.3){}; %Empty Node
% \node (D3) at (11.5,-3.3){}; %Empty Node
% \node (D4) at (13.5,-3.3){}; %Empty Node
% \end{tikzpicture}

\begin{tikzpicture}[scale=0.7, every node/.style={scale=0.7}]
%\draw(1.5,0.2);
\draw(2,2.2) node{$D_1$};
\draw(6,2.2) node{$D_2$};
\draw(10,2.2) node{$D_3$};
\draw(14,2.2) node{$D_4$};
\draw(18,2.2) node{$D_5$};

\draw (0.5,2) rectangle (3.4,-4.5);
\draw (4.5,2) rectangle (7.4,-4.5);
\draw (8.5,2) rectangle (11.4,-4.5);
\draw (12.5,2) rectangle (15.4,-4.5);
\draw (16.5,2) rectangle (19.4,-4.5);

\draw[radius=0.4mm, color=black, fill=black](1,-4) circle node[anchor=north east]{1};
\draw[radius=0.4mm, color=black, fill=black](2,-4) circle node[below=0.02cm]{2};
\draw[radius=0.4mm, color=black, fill=black](3,-4) circle node[below=0.02cm]{3} node[above=0.02cm] {$z_1$};
\draw[radius=0.4mm, color=black, fill=black](4,-4) circle node[below=0.02cm]{4};
\draw[radius=0.4mm, color=black, fill=black](5,-4) circle node[below=0.02cm] {5};
\draw[radius=0.4mm, color=black, fill=black](6,-4) circle node[below=0.02cm]{6}  node[above=0.02cm] {$z_2$}; 
\draw[radius=0.4mm, color=black, fill=black](7,-4) circle node[below=0.02cm]{7};
\draw[radius=0.4mm, color=black, fill=black](8,-4) circle node[below=0.02cm]{8};
\draw[radius=0.4mm, color=black, fill=black](9,-4) circle node[anchor=north east]{9};
\draw[radius=0.4mm, color=black, fill=black](10,-4) circle node[below=0.02cm]{10} node[above=0.02cm] {$z_3$};
\draw[radius=0.4mm, color=black, fill=black](11,-4) circle node[below=0.02cm]{11};
\draw[radius=0.4mm, color=black, fill=black](12,-4) circle node[below=0.02cm]{12};
\draw[radius=0.4mm, color=black, fill=black](13,-4) circle node[below=0.02cm]{13};
\draw[radius=0.4mm, color=black, fill=black](14,-4) circle node[below=0.02cm]{14} node[above=0.02cm] {$z_4$};
\draw[radius=0.4mm, color=black, fill=black](15,-4) circle node[below=0.02cm]{15};
\draw[radius=0.4mm, color=black, fill=black](16,-4) circle node[below=0.02cm]{16};
\draw[radius=0.4mm, color=black, fill=black](17,-4) circle node[below=0.02cm]{17};
\draw[radius=0.4mm, color=black, fill=black](18,-4) circle node[anchor=north east]{18} node[anchor=south west] {$z_5$};
\draw[radius=0.4mm, color=black, fill=black](19,-4) circle node[below=0.02cm]{19};

\draw[dashed](1,-4)--(19,-4); 

\draw(3,1)--(14,1); %I_u
\draw(2,0)--(10,0); %I_a
\draw(10,-1)--(18,-1); %I_b
\draw(1,-1)--(6,-1); %I_d
\draw(6,-2)--(11,-2); %I_e 
\draw(9,-3)--(15,-3); %I_c
\draw(18,0)--(19,0); %I_f

\draw[radius=0.2mm, fill=black](3,1) circle node[above=0.02cm] {$I_u$};
\draw[radius=0.2mm, fill=black](14,1) circle;
\draw[radius=0.2mm, fill=black](2,0) circle node[above=0.02cm] {$I_a$};
\draw[radius=0.2mm, fill=black](10,0) circle;
\draw[radius=0.2mm, fill=black](2,-1) circle node[above=0.02cm] {$I_d$};
\draw[radius=0.2mm, fill=black](6,-1) circle;
\draw[radius=0.2mm, fill=black](10,-1) circle node[above=0.02cm] {$I_b$};
\draw[radius=0.2mm, fill=black](18,-1) circle;
\draw[radius=0.2mm, fill=black](6,-2) circle node[above=0.02cm] {$I_e$};
\draw[radius=0.2mm, fill=black](11,-2) circle;
\draw[radius=0.2mm, fill=black](10,-3) circle node[above=0.02cm] {$I_c$};
\draw[radius=0.2mm, fill=black](15,-3) circle;
\draw[radius=0.2mm, fill=black](19,0) circle node[above=0.02cm] {$I_f$};
\draw[radius=0.2mm, fill=black](19,0) circle;

\draw(2,-5.5) node{$K_1$};
\draw(10,-5.5) node{$K_2$};
\draw(18,-5.5) node{$K_3$};

\draw[dashed](1,1.5)--(1,-5); % EHS point 1
\draw[dashed](9,1.5)--(9,-5); % EHS point 9
\draw[dashed](18,1.5)--(18,-5); % EHS point 18
\end{tikzpicture}

\caption{\scriptsize{Exact hitting set is \{1,9,18\}}}
\label{fig:gadgetAndMinClique}
\end{figure}%

